Generating Special Triangulations with Transformers

Triangulations, i.e., well-structured decompositions of geometric objects into triangle-like pieces, are central objects in many domains of mathematics and physics. In particular, fine, regular, and star triangulations (FRSTs) of 4D reflexive polytopes give rise to smooth Calabi-Yau threefolds, which are of significant interest in string theory. However, the high dimensionality and combinatorial complexity of triangulations make them particularly challenging to model with classical numerical methods or machine learning. In this work, we show that transformers, equipped with an appropriate encoding scheme, can be effectively trained to representatively generate new FRSTs across a range of polytope sizes. Moreover, these models can also self-improve through retraining on their own output. This opens the door to both concrete applications to the classification of Calabi-Yau manifolds and further research in physics, combinatorics and algebraic geometry.

==> plots/full_architecture.tex <==
\begin{tikzpicture}[
    >=Latex, thick,
    encoder/.style={
        draw=blue!50, fill=blue!15, rounded corners=8pt,
        minimum width=3.5cm, minimum height=2.5cm, align=center
    },
    decoder/.style={
        draw=orange!70!red, fill=orange!20, rounded corners=8pt,
        minimum width=3.5cm, minimum height=2.5cm, align=center
    },
    io/.style={font=\small, align=center}
  ]

  % Nodes
  \node[encoder] (enc) at (0,0) {Encoder};
  \node[decoder] (dec) at (7,0) {Decoder};

  % Input vectors and dots
  \node[io] (enc_in) at (0,-3.5) {%
    $\displaystyle
    \begin{bmatrix} -1 \\ 0 \\ 0 \\ 0 \end{bmatrix}
    \quad
    \cdots
    \quad
    \begin{bmatrix} -1 \\ 1 \\ -1 \\ 0 \end{bmatrix}
    $};

  % Legend (adjusted slightly upward)
  \node[io, below=0cm of enc_in] (legend) {Input polytope};

  % Coordinates for the left and right ends of the input group
  \coordinate (in_left) at ($(enc_in.west) + (0,1.0)$);
  \coordinate (in_right) at ($(enc_in.east) + (0,1.0)$);

  % Brace decoration above the vectors
  \draw[decorate,decoration={brace,amplitude=6pt},thick]
    (in_left) -- (in_right);

% Encoder output (vertical dots in vectors)
\node[io, above=0.75cm of enc] (enc_out) {%
  $\displaystyle
\scalebox{1.2}{$\begin{bmatrix} \phantom{0} \\ \vdots \\ \phantom{0} \end{bmatrix}$}
    \quad
    \cdots
    \quad
    \scalebox{1.2}{$\begin{bmatrix} \phantom{0} \\ \vdots \\ \phantom{0} \end{bmatrix}$}
  $
};

  % Legend above encoder output
  \node[io, above=0.cm of enc_out] {Encoder output};


    % Legend below the token sequence
  \node[io, below=1.5cm of dec] (dec_in) {%
  $\langle \text{sos} \rangle \;\; \langle 20 \rangle \;\; \langle 32 \rangle \;\; \langle 90 \rangle \;\; \text{ \large\textcolor{red}{ ?}}$
};

 \node[io, below=0.0cm of dec_in] {Partially constructed sequence of tokens};

 % Coordinates for the left and right ends of the input group
  \coordinate (in_dec_left) at ($(dec_in.west) + (0,0.5)$);
  \coordinate (in_dec_right) at ($(dec_in.east) + (0,0.5)$);

  % Brace decoration above the vectors
  \draw[decorate,decoration={brace,amplitude=6pt},thick]
    (in_dec_left) -- (in_dec_right);

  \node[io, above=0.75cm of dec] (dec_out) {%
  $P = \left[ p_1, \dots, p_M \right]$
};

  \node[io, above=0.0cm of dec_out] {%
  Probability distribution\\
  over tokens
};

% Token node to the right of final output
\node[io, right=2.2cm of dec_out] (sampled_token) {%
  $\langle 34 \rangle$
};

\node[io, above=0.0cm of sampled_token] {%
  New token
};

% Arrow from final output to sampled token
\draw[->, thick] (dec_out) -- (sampled_token);

% Legend below the arrow
\node[io, below=0.0cm of $(dec_out)!0.5!(sampled_token)$] {sampling};

  % Arrow from vectors to encoder
  \draw[->, thick] ($(enc_in.north) + (0,0.45)$) -- ($(enc.south) + (0,-0.1)$);

  % Arrow path from encoder output to decoder input
  \coordinate (p1) at ($(enc_out) + (2.5,0)$);
  \coordinate (p2) at ($(p1) + (0,-5)$);
  \coordinate (p3) at ($(p2) + (4,0)$);
  \coordinate (dec_enc_point) at ($(dec.south) + (-0.5,0)$);

  % Other arrows
  \draw[->, thick] (enc) -- (enc_out);
  \draw[->, thick] ($(dec_in.north) + (0,0.55)$) -- (dec.south);
  \draw[->, thick] (dec) -- (dec_out);

  % Rounded arrow from encoder output to decoder input
  \draw[->, thick, rounded corners=8pt]
    (enc_out) -- (p1) -- (p2) -- (p3) -- (dec_enc_point);

% Define intermediate points for rounded arrow from sampled_token to dec_in
\coordinate (s1) at ($(sampled_token) + (0,-1.5)$);  % down

% Extract x from s1 and y from dec_in.east to define s2
\path let \p1 = (s1), \p2 = (dec_in.east) in
  coordinate (s2) at (\x1, \y2);

% Coordinate for the entry point to dec_in
\coordinate (dec_in_right) at (dec_in.east);

% Draw the arrow
\draw[->, thick, rounded corners=8pt]
  (sampled_token) -- (s1) -- (s2) -- (dec_in_right);

\end{tikzpicture}
